Generalised Gaussian Process Latent Variable Models (GPLVM) with Stochastic Variational Inference

Gaussian process latent variable models (GPLVM) are a flexible and non-linear approach to dimensionality reduction, extending classical Gaussian processes to an unsupervised learning context. The Bayesian incarnation of the GPLVM Titsias and Lawrence, 2010] uses a variational framework, where the posterior over latent variables is approximated by a well-behaved variational family, a factorized Gaussian yielding a tractable lower bound. However, the non-factories ability of the lower bound prevents truly scalable inference. In this work, we study the doubly stochastic formulation of the Bayesian GPLVM model amenable with minibatch training. We show how this framework is compatible with different latent variable formulations and perform experiments to compare a suite of models. Further, we demonstrate how we can train in the presence of massively missing data and obtain high-fidelity reconstructions. We demonstrate the model's performance by benchmarking against the canonical sparse GPLVM for high-dimensional data examples.

==> graphs/old/model_pca.tex <==

% model_pca.tex
%
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes
  \node[obs]                               (y) {$y$};
  \node[latent, above=of y, xshift=-1.2cm] (w) {$\mathbf{w}$};
  \node[latent, above=of y, xshift=1.2cm]  (x) {$\mathbf{x}$};
  \node[latent, right=2cm of y]            (t) {$\tau$};

  % Connect the nodes
  \edge {x,w,t} {y} ; %

  % Plates
  \plate {yx} {(x)(y)} {$N$} ;
  \plate {} {(w)(y)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End:

==> graphs/old/model_pca2.tex <==
% model_pca2.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes

  % Y
  \node[obs]          (y)   {$y$}; %
  \factor[above=of y] {y-f} {left:$\mathcal{N}$} {} {} ; %

  % W and X
  \node[det, above=of y]            (dot) {dot} ; % 
  \node[latent, above left=1.2 of dot]  (w)   {$\mathbf{w}$}; %
  \node[latent, above right=1.2 of dot] (x)   {$\mathbf{x}$}; %

  % W hyperparameters
  \node[const, above=1.2 of w, xshift=-0.5cm] (mw) {$\mu_w$} ; %
  \node[const, above=1.2 of w, xshift=0.5cm]  (aw) {$\alpha_w$} ; %

  % X hyperparameters
  \node[const, above=1.2 of x, xshift=-0.5cm] (mx) {$\mu_x$} ; %
  \node[const, above=1.2 of x, xshift=0.5cm]  (ax) {$\alpha_x$} ; %

  % noise
  \node[latent, right=2.5cm of y-f]         (t)   {$\tau$}; %
  \node[const, above=of t, xshift=-0.5cm] (at)  {$\alpha_\tau$} ; %
  \node[const, above=of t, xshift=0.5cm]  (bt)  {$\beta_\tau$} ; %

  % Factors
  \factor[above=of w] {w-f} {left:$\mathcal{N}$} {mw,aw} {w} ; %
  \factor[above=of x] {x-f} {left:$\mathcal{N}$} {mx,ax} {x} ; %
  \factor[above=of t] {t-f} {left:$\mathcal{G}$} {at,bt} {t} ; %
  \factoredge {dot,t} {y-f} {y} ; %

  % Connect w and x to the dot node
  \edge[-] {w,x} {dot} ;

  % Plates
  \plate {yx} { %
    (y)(y-f)(y-f-caption) %
    (x)(x-f)(x-f-caption) %
    (dot) %
  } {$N$} ;
  \plate {} {%
    (y)(y-f)(y-f-caption) %
    (w)(w-f)(w-f-caption) %
    (dot) %
    (yx.north west)(yx.south west) %
  } {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
